Can We Identify Stack Overflow Questions Requiring Code Snippets? Investigating the Cause & Effect of Missing Code Snippets

On the Stack Overflow (SO) Q&A site, users often request solutions to their code-related problems (e.g., errors, unexpected behavior). Unfortunately, they often miss required code snippets during their question submission, which could prevent their questions from getting prompt and appropriate answers. In this study, we conduct an empirical study investigating the cause & effect of missing code snippets in SO questions whenever required. Here, our contributions are threefold. First, we analyze how the presence or absence of required code snippets affects the correlation between question types (missed code, included code after requests & had code snippets during submission) and corresponding answer meta-data (e.g., presence of an accepted answer). According to our analysis, the chance of getting accepted answers is three times higher for questions that include required code snippets during their question submission than those that missed the code. We also investigate whether the confounding factors (e.g., user reputation) affect questions receiving answers besides the presence or absence of required code snippets. We found that such factors do not hurt the correlation between the presence or absence of required code snippets and answer meta-data. Second, we surveyed 64 practitioners to understand why users miss necessary code snippets. About 60% of them agree that users are unaware of whether their questions require any code snippets. Third, we thus extract four text-based features (e.g., keywords) and build six ML models to identify the questions that need code snippets. Our models can predict the target questions with 86.5% precision, 90.8% recall, 85.3% F1-score, and 85.2% overall accuracy. Our work has the potential to save significant time in programming question-answering and improve the quality of the valuable knowledge base by decreasing unanswered and unresolved questions.

==> Notes.tex <==

Total questions (March 2020): 18714405

Total questions: 20974 (matched key-phrases with comments)
Code after comment (has code): 14935



*************** Findings ***********************

> After comments, many users added their code segments, such findings motivate us to introduce a tool that will detect questions that require code segments. 

> Someone add code or image of the code, then the question got answer, then by editing question submitter remove the code. So, finally, the question has no code, however, the question had code for a period.

> We can see how many accepted answers were submitted before adding code. We also can analyze the answer quality submitted before and after the code inclusion.

> Looks like comment and code submission delay is important. Long delay might prevent questions from receiving answers. Need to immediately follow the comments.

> Submitted an answer, after including the code to question, answer was also edited, then accepted. It clearly indicates that it is not possible to answer properly with appropriate code examples.

> We should have filtered the questions whose last edited time is not NULL. We found some questions that were not edited at all.

>> Need to check what percentage of accepted/best answers were submitted before and after adding code

>> Some answer are edited after submitted code, and then accepted as working solution. That means, without code developers answer question by guessing sometimes.

>> How many answers were accepted that were submitted before adding code?

>> Time zone is different, so question submitter did not follow the comments immediately after the comments. (e.g., comments out of official period or sleeping time). Opposite is also true, when question submitter added code, the developer who intended to answer become unavailable. Moreover, others can edit questions to improve other quality (e.g., presentation, grammar), but they could not add the appropriate code examples, only the question submitters can do it.

     **Case: When added code after long gap, many questions did not receive acceptable answers.
     
>> Sometimes a solution accepted by the question submitter before adding code. However, answer submitted after adding code becomes best answer, that mean, a answer with highest positive votes.

>> Added code, later deleted. It refers that the added code segment was not appropriate.

>> Observation: The questions that did not receive answer even after adding code upon request, the time difference between comment and code addition is too high. 

>> For the dataset where user added code during question submission: We check whether user submit real code or not in the initial version of question. Sometimes code is added later by editing, sometimes error message, input values are added under <pre> tag. In particular, we see is there any real code in the initial version of the question.

>> Find best answer or accepted answer score

>> We will provide statistics with the tool message. For example, if you do not add code example, you have only x\% possibility to receive acceptable answer.

Discourse Analysis
--------------------

>> Text has code elements
>> Find programming activity (What actually programming does!!)
>> Sentences include "BUT/HOWEVER/EXCEPT/WHILE" represents unexpected behaviour/discrepancy/deviation.


>> Positive clause + "BUT/HOWEVER/EXCEPT/WHILE/WHEN/BECAUSE" + negative clause OR vice versa
>> Positive sentence + "BUT/HOWEVER/EXCEPT/WHILE" + negative sentence OR vice versa
>> I am new + preposition + programming language
>> Camel case words in the title
>> Start title with verb/gerund

>> Check how many questions that do not need code has inline code element. Then we could claim that "having code element indicates that discussing code related issues"

>> Labeled the keywords and the key phrases and sentences.

>> Number of code elements can be a feature 
>> Target keywords, get context (a few words before and a few words after), then check them whether we can find any rules

Note: sorry for not having actual code, then tool should not ask code. If there is info such as "code is proprietary", then tool also should not ask for code.



POS Tagging
--------------------------------------------------
>> Title of the questions with no code: WP: 11%
>> Title of the questions with code: WP: 1%
>> "WRB TO" is frequent in the questions with code.

>> "PRP VBP VBG TO VB" frequent in the questions having code

>> "NN CC WRB PRP VBP" frequent in the questions having code

>> First sentence of the body contains "I am trying.." "I am implementing.."

Treat to validity: We get the edit approved time, not the edit time when the edits are reviewed by experts.


Who miss the code segments frequently, new, low-reputed, ....?



>> To find the empirical evidence, we attempt to find three types of questions: miss code snippets, submit code snippets after request, and included code during submission.

>> To find the questions that miss the code snippets, we search a few key phrases in the comments that asked for code snippets, but the questions did not have any code snippets.

>> For the second category, we search the key phrases and check the questions were edited and had code snippets.

>> For the third category, no edit, have code snippets..................

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?
A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets.

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?

A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets. Additionally, some users may not be familiar with the syntax and formatting of code snippets, or may not be aware of the best practices for including them in their questions.

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?
A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets. Additionally, some users may not be familiar with the syntax and formatting of code snippets or may not be aware of the best practices for including them in their questions. Additionally, some users

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?
A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets. Additionally, some users may not be familiar with the syntax and formatting of code snippets or may not be aware of the best practices for including them in their questions. Additionally, some users

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?
A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets. Additionally, some users may not be familiar with the syntax and formatting of code snippets or may not be aware of the best practices for including them in their questions. Additionally, some users

Q: Why do Stack Overflow users miss adding code snippets to their questions whenever required?
A: Stack Overflow users may miss adding code snippets to their questions for a variety of reasons. Some users may not be aware of the importance of including code snippets, while others may not have the technical knowledge to include them. Additionally, some users may be in a hurry and not take the time to include code snippets. Additionally, some users may not be familiar with the syntax and formatting of code snippets, or may not be aware of the best practices for including them in their questions. Additionally, some users

==> boxplot-acc-ans-score.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%
        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {Score},
          xtick = {1, 2, 3},
          xticklabels = {MICO, COAC, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        -1\\
        -2\\
        -1\\
        1\\
        1\\
        0\\
        -3\\
        -1\\
        2\\
        -2\\
        2\\
        1\\
        0\\
        -1\\
        1\\
        0\\
        2\\
        3\\
        1\\
        2\\
        1\\
        -1\\
        0\\
        3\\
        1\\
        0\\
        1\\
        0\\
        -2\\
        0\\
        2\\
        -2\\
        0\\
        1\\
        4\\
        -2\\
        0\\
        0\\
        0\\
        3\\
        0\\
        -1\\
        2\\
        7\\
        0\\
        1\\
        -4\\
        1\\
        0\\
        0\\
        0\\
        2\\
        1\\
        1\\
        0\\
        0\\
        0\\
        -1\\
        -1\\
        -1\\
        -7\\
        -2\\
        0\\
        0\\
        3\\
        0\\
        0\\
        -1\\
        5\\
        2\\
        -3\\
        -1\\
        -2\\
        -1\\
        1\\
        -5\\
        0\\
        0\\
        -1\\
        0\\
        0\\
        0\\
        1\\
        -3\\
        -1\\
        1\\
        0\\
        1\\
        1\\
        0\\
        0\\
        -6\\
        6\\
        1\\
        0\\
        };
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            10\\
            8\\
            0\\
            1\\
            0\\
            1\\
            12\\
            0\\
            0\\
            1\\
            1\\
            7\\
            3\\
            -1\\
            0\\
            1\\
            1\\
            0\\
            0\\
            9\\
            0\\
            1\\
            0\\
            5\\
            1\\
            -2\\
            1\\
            0\\
            1\\
            3\\
            0\\
            1\\
            -5\\
            0\\
            1\\
            -3\\
            2\\
            2\\
            4\\
            0\\
            -1\\
            1\\
            8\\
            -2\\
            -1\\
            0\\
            2\\
            0\\
            0\\
            1\\
            2\\
            0\\
            0\\
            2\\
            2\\
            4\\
            1\\
            -1\\
            2\\
            -2\\
            1\\
            0\\
            1\\
            0\\
            0\\
            1\\
            2\\
            1\\
            1\\
            4\\
            0\\
            0\\
            0\\
            5\\
            0\\
            0\\
            2\\
            0\\
            -1\\
            1\\
            1\\
            0\\
            2\\
            0\\
            0\\
            2\\
            0\\
            1\\
            -2\\
            2\\
            -1\\
            -2\\
            0\\
            1\\
            22\\
            0\\
            2\\
            0\\
            0\\
            1\\
            -1\\
            -1\\
            -5\\
            1\\
            0\\
            -1\\
            0\\
            1\\
            -1\\
            0\\
            1\\
            4\\
            0\\
            0\\
            0\\
            0\\
            1\\
            0\\
            0\\
            0\\
            1\\
            9\\
            0\\
            -1\\
            1\\
            1\\
            0\\
            0\\
            0\\
            -2\\
            0\\
            0\\
            4\\
            -1\\
            -1\\
            -1\\
            -1\\
            1\\
            0\\
            -3\\
            0\\
            0\\
            0\\
            1\\
            2\\
            1\\
            0\\
            1\\
            0\\
            2\\
            0\\
            0\\
            0\\
            9\\
            1\\
            -1\\
            0\\
            1\\
            3\\
            1\\
            0\\
            0\\
            0\\
            2\\
            -2\\
            1\\
            0\\
            0\\
            0\\
            };
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        13\\
        1\\
        35\\
        73\\
        8\\
        3\\
        14\\
        13\\
        4\\
        2\\
        4\\
        7\\
        169\\
        10\\
        13\\
        12\\
        5\\
        7\\
        2\\
        582\\
        1\\
        803\\
        187\\
        97\\
        334\\
        10\\
        5\\
        0\\
        71\\
        24\\
        13\\
        21\\
        20\\
        14\\
        47\\
        346\\
        11\\
        4\\
        49\\
        13\\
        32\\
        41\\
        6\\
        1\\
        16\\
        15\\
        18\\
        4\\
        6\\
        1\\
        6\\
        -3\\
        0\\
        12\\
        1\\
        4\\
        6\\
        0\\
        1\\
        0\\
        2\\
        3\\
        3\\
        4\\
        1\\
        0\\
        6\\
        1\\
        0\\
        0\\
        1\\
        2\\
        0\\
        0\\
        0\\
        0\\
        33\\
        3\\
        0\\
        0\\
        2\\
        4\\
        0\\
        7\\
        5\\
        3\\
        8\\
        6\\
        1\\
        11\\
        0\\
        0\\
        8\\
        1\\
        5\\
        3\\
        1\\
        1\\
        0\\
        1\\
        2\\
        1\\
        0\\
        0\\
        1\\
        0\\
        0\\
        3\\
        0\\
        2\\
        6\\
        0\\
        15\\
        0\\
        0\\
        0\\
        25\\
        0\\
        4\\
        19\\
        1\\
        10\\
        0\\
        0\\
        0\\
        1\\
        1\\
        2\\
        2\\
        8\\
        1\\
        5\\
        0\\
        1\\
        2\\
        1\\
        4\\
        2\\
        11\\
        1\\
        2\\
        0\\
        0\\
        68\\
        3\\
        0\\
        0\\
        1\\
        1\\
        13\\
        2\\
        1\\
        16\\
        0\\
        6\\
        0\\
        3\\
        1\\
        0\\
        0\\
        1\\
        0\\
        0\\
        0\\
        0\\
        2\\
        0\\
        0\\
        9\\
        -2\\
        0\\
        0\\
        1\\
        0\\
        3\\
        0\\
        6\\
        1\\
        19\\
        0\\
        -1\\
        0\\
        3\\
        0\\
        3\\
        0\\
        0\\
        1005\\
        1\\
        4\\
        12\\
        0\\
        4\\
        6\\
        2\\
        -5\\
        0\\
        4\\
        0\\
        5\\
        4\\
        63\\
        2\\
        0\\
        1\\
        -2\\
        2\\
        0\\
        2\\
        3\\
        0\\
        0\\
        1\\
        0\\
        3\\
        0\\
        1\\
        7\\
        1\\
        1\\
        1\\
        1\\
        3\\
        0\\
        0\\
        1\\
        5\\
        1\\
        1\\
        0\\
        0\\
        -1\\
        0\\
        -1\\
        1\\
        2\\
        -1\\
        -1\\
        0\\
        1\\
        1\\
        0\\
        2\\
        -2\\
        0\\
        3\\
        0\\
        0\\
        0\\
        1\\
        };
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Score of accepted answer (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:score-acc-ans}
\end{figure}

==> boxplot-delay-adding-code.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {Time delay (in minutes)},
          xtick = {1, 2, 3},
          xticklabels = {No Answer, Unresolved, Resolved},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        34\\
        5\\
        6\\
        609\\
        8\\
        38\\
        21\\
        799\\
        38\\
        2\\
        728\\
        16\\
        10\\
        32\\
        4\\
        799\\
        13\\
        1\\
        975\\
        7\\
        1403\\
        15\\
        84\\
        2023\\
        15\\
        16\\
        20\\
        1172\\
        1249\\
        2370\\
        865\\
        1\\
        2\\
        4351\\
        15\\
        13\\
        9\\
        456\\
        4\\
        6\\
        1412\\
        100\\
        10\\
        398\\
        2975\\
        35\\
        15\\
        17\\
        134\\
        17\\
        991\\
        23\\
        16\\
        1086\\
        7\\
        310\\
        2\\
        2512\\
        52\\
        835\\
        12\\
        49\\
        20\\
        7\\
        9006\\
        1879\\
        12\\
        3\\
        913\\
        1847\\
        5\\
        10\\
        885\\
        942\\
        11\\
        7\\
        9\\
        24\\
        10\\
        144\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            0\\
            0\\
            0\\
            0\\
            1\\
            1\\
            1\\
            1\\
            1\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            5\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            6\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            7\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            8\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            9\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            10\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            11\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            12\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            13\\
            14\\
            14\\
            14\\
            15\\
            15\\
            15\\
            15\\
            15\\
            15\\
            15\\
            16\\
            16\\
            16\\
            17\\
            17\\
            17\\
            17\\
            18\\
            18\\
            20\\
            20\\
            20\\
            20\\
            20\\
            21\\
            21\\
            22\\
            22\\
            22\\
            22\\
            22\\
            22\\
            22\\
            23\\
            23\\
            23\\
            23\\
            23\\
            23\\
            25\\
            25\\
            25\\
            26\\
            26\\
            26\\
            26\\
            27\\
            28\\
            28\\
            28\\
            29\\
            29\\
            29\\
            30\\
            30\\
            31\\
            31\\
            32\\
            32\\
            32\\
            32\\
            32\\
            33\\
            33\\
            35\\
            36\\
            36\\
            36\\
            39\\
            39\\
            40\\
            40\\
            41\\
            43\\
            43\\
            44\\
            44\\
            45\\
            46\\
            49\\
            49\\
            50\\
            50\\
            51\\
            51\\
            51\\
            54\\
            55\\
            59\\
            60\\
            60\\
            61\\
            63\\
            68\\
            69\\
            77\\
            80\\
            83\\
            83\\
            87\\
            93\\
            95\\
            107\\
            109\\
            115\\
            136\\
            146\\
            147\\
            155\\
            157\\
            160\\
            160\\
            162\\
            169\\
            172\\
            184\\
            206\\
            209\\
            215\\
            216\\
            219\\
            229\\
            231\\
            232\\
            243\\
            355\\
            376\\
            447\\
            456\\
            496\\
            502\\
            701\\
            745\\
            843\\
            959\\
            994\\
            999\\
            1069\\
            1070\\
            1076\\
            1158\\
            1274\\
            1321\\
            1450\\
            1585\\
            1609\\
            1680\\
            1688\\
            1918\\
            2540\\
            2721\\
            3843\\
            5060\\
            5317\\
            5714\\
            8244\\
            18786\\
            };
            
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            2\\
            355\\
            447\\
            21\\
            10\\
            7\\
            2\\
            29\\
            95\\
            5\\
            25\\
            1609\\
            4\\
            4\\
            61\\
            8\\
            6\\
            44\\
            50\\
            8\\
            206\\
            12\\
            11\\
            9\\
            35\\
            7\\
            10\\
            9\\
            0\\
            7\\
            1\\
            8\\
            6\\
            2\\
            7\\
            209\\
            115\\
            4\\
            14\\
            157\\
            5\\
            10\\
            160\\
            36\\
            51\\
            8\\
            11\\
            20\\
            6\\
            0\\
            1\\
            14\\
            83\\
            15\\
            1076\\
            17\\
            376\\
            15\\
            0\\
            5\\
            16\\
            6\\
            17\\
            68\\
            60\\
            26\\
            16\\
            28\\
            12\\
            4\\
            22\\
            26\\
            3\\
            30\\
            12\\
            5\\
            12\\
            155\\
            11\\
            1918\\
            229\\
            5\\
            22\\
            5\\
            7\\
            11\\
            6\\
            10\\
            31\\
            29\\
            843\\
            10\\
            5714\\
            8\\
            1585\\
            2\\
            22\\
            26\\
            15\\
            5060\\
            41\\
            49\\
            8\\
            2\\
            27\\
            4\\
            1\\
            2\\
            9\\
            3\\
            20\\
            2\\
            3\\
            3\\
            10\\
            80\\
            22\\
            502\\
            959\\
            33\\
            701\\
            11\\
            4\\
            172\\
            232\\
            43\\
            2\\
            18\\
            8\\
            1069\\
            5\\
            4\\
            1\\
            5\\
            7\\
            2\\
            20\\
            3\\
            51\\
            60\\
            21\\
            23\\
            8\\
            6\\
            0\\
            4\\
            15\\
            7\\
            2721\\
            3\\
            4\\
            14\\
            8\\
            39\\
            13\\
            20\\
            4\\
            3\\
            11\\
            10\\
            87\\
            3\\
            31\\
            51\\
            25\\
            6\\
            10\\
            40\\
            18\\
            5\\};
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Time delay between comment \& code addition by editing.}
% \vspace{-3mm}
\label{fig:time-delay-adding-code}
\end{figure}

==> boxplot-number-of-answers.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3in,height=3in,
          ylabel = {\# of answers},
          xtick = {1, 2, 3},
          xticklabels = {MICO, COAC, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        0\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        1\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        3\\
        4\\
        4\\
        4\\
        4\\};
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            0\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            1\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            2\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            3\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            4\\
            5\\
            5\\
            5\\
            6\\
            8\\
            };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        3\\
        10\\
        10\\
        2\\
        16\\
        7\\
        16\\
        10\\
        5\\
        5\\
        2\\
        1\\
        6\\
        6\\
        5\\
        6\\
        14\\
        14\\
        4\\
        13\\
        8\\
        2\\
        1\\
        5\\
        3\\
        26\\
        2\\
        50\\
        13\\
        10\\
        16\\
        2\\
        2\\
        1\\
        3\\
        7\\
        6\\
        5\\
        2\\
        7\\
        2\\
        2\\
        4\\
        10\\
        2\\
        1\\
        1\\
        9\\
        0\\
        1\\
        1\\
        3\\
        3\\
        4\\
        4\\
        3\\
        4\\
        1\\
        3\\
        1\\
        3\\
        3\\
        0\\
        4\\
        2\\
        2\\
        1\\
        1\\
        2\\
        1\\
        0\\
        1\\
        4\\
        4\\
        2\\
        2\\
        3\\
        3\\
        3\\
        1\\
        1\\
        1\\
        0\\
        1\\
        1\\
        2\\
        1\\
        1\\
        4\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        2\\
        2\\
        1\\
        0\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        3\\
        2\\
        0\\
        1\\
        2\\
        5\\
        1\\
        2\\
        1\\
        1\\
        0\\
        1\\
        0\\
        2\\
        1\\
        1\\
        1\\
        1\\
        4\\
        1\\
        3\\
        0\\
        0\\
        2\\
        2\\
        0\\
        1\\
        0\\
        1\\
        7\\
        2\\
        4\\
        3\\
        3\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        2\\
        1\\
        1\\
        3\\
        0\\
        3\\
        0\\
        4\\
        0\\
        2\\
        1\\
        1\\
        2\\
        1\\
        1\\
        3\\
        3\\
        2\\
        2\\
        1\\
        1\\
        3\\
        1\\
        3\\
        1\\
        1\\
        1\\
        4\\
        1\\
        1\\
        2\\
        1\\
        2\\
        2\\
        3\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        0\\
        2\\
        2\\
        1\\
        2\\
        2\\
        1\\
        2\\
        1\\
        1\\
        7\\
        0\\
        1\\
        1\\
        1\\
        1\\
        4\\
        2\\
        2\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        5\\
        3\\
        1\\
        0\\
        3\\
        4\\
        1\\
        2\\
        1\\
        1\\
        1\\
        1\\
        3\\
        1\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        3\\
        5\\
        1\\
        1\\
        3\\
        2\\
        1\\
        2\\
        1\\
        12\\
        3\\
        2\\
        1\\
        1\\
        4\\
        1\\
        1\\
        1\\
        5\\
        1\\
        2\\
        1\\
        2\\
        1\\
        0\\
        1\\
        2\\
        1\\
        1\\
        3\\
        0\\
        2\\
        2\\
        1\\
        2\\
        5\\
        2\\
        1\\
        2\\
        1\\
        4\\
        0\\
        2\\
        1\\
        1\\
        1\\
        1\\
        7\\
        1\\
        1\\
        1\\
        2\\
        1\\
        0\\
        1\\
        2\\
        3\\
        2\\
        2\\
        1\\
        1\\
        4\\
        1\\
        2\\
        3\\
        3\\
        2\\
        2\\
        2\\
        2\\
        2\\
        2\\
        1\\
        9\\
        1\\
        3\\
        4\\
        2\\
        1\\
        1\\
        7\\
        1\\
        2\\
        1\\
        1\\
        1\\
        2\\
        1\\
        2\\
        6\\
        2\\
        4\\
        1\\
        1\\
        2\\
        1\\
        2\\
        0\\
        1\\
        0\\
        1\\
        0\\
        1\\
        1\\
        1\\
        2\\
        1\\
        1\\
        1\\
        3\\
        1\\
        1\\
        0\\
        2\\
        1\\
        0\\
        1\\
        3\\
        1\\
        4\\
        2\\
        0\\
        2\\
        1\\
        1\\
        2\\
        1\\
        3\\
        2\\
        2\\
        1\\
        0\\
        1\\
        2\\
        0\\
        1\\
        1\\
        1\\
        1\\
        3\\
        1\\
        2\\
        2\\
        3\\
        1\\
        3\\
        2\\
        1\\
        3\\
        2\\
        2\\
        1\\
        1\\
        1\\
        1\\
        3\\
        3\\
        1\\
        1\\
        2\\
        4\\
        3\\
        1\\
        1\\
        1\\
        1\\
        2\\
        1\\
        2\\
        2\\
        2\\
        };
        
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Number of answers (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:no-of-answers}
\end{figure}

==> boxplot-time-delay-receiving-acc-ans.tex <==

\begin{figure}[!htp]
\centering
        \resizebox{3.3in}{!}{%

        \begin{tikzpicture}
        \begin{axis}[xmin=0,width=3.5in,height=3.5in,
          ylabel = {Time delay (in minutes)},
          xtick = {1, 2, 3, 4},
          xticklabels = {MICO, COAC, COAC*, CODS},
          %every axis plot/.append style = {fill, fill opacity = .1}
          ]
        % somewhen the simple statement of `hide outliers` broke.
        % Now the full path to the style needs to be written.
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.0,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        83\\
        496\\
        7\\
        542\\
        169\\
        849\\
        29\\
        30\\
        47\\
        41\\
        20\\
        29\\
        3\\
        2\\
        96\\
        568\\
        3358\\
        1072\\
        45\\
        217144\\
        4535\\
        9\\
        106\\
        123941\\
        80\\
        3\\
        214\\
        1235\\
        10\\
        418\\
        217\\
        42\\
        51\\
        143\\
        11459\\
        104\\
        446\\
        41\\
        191\\
        155\\
        10416\\
        40\\
        1645\\
        42\\
        6\\
        2369\\
        10\\
        61\\
        1065\\
        22\\
        159\\
        17\\
        663\\
        29\\
        711\\
        1650\\
        74\\
        30\\
        1\\
        24\\
        10\\
        9825\\
        41\\
        71\\
        191\\
        48\\
        62\\
        5\\
        232\\
        4\\
        5\\
        17\\
        28\\
        14\\
        35\\
        23\\
        35\\
        106200\\
        433\\
        7\\
        576472\\
        185\\
        4\\
        26\\
        4\\
        386\\
        4155\\
        38\\
        39\\
        5\\
        461\\
        15\\
        13\\
        28\\
        73\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.1,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        248\\
        79\\
        125\\
        5209\\
        42\\
        80\\
        529\\
        6028\\
        1140\\
        30\\
        54\\
        170\\
        3185\\
        317\\
        13\\
        68\\
        33\\
        5\\
        19\\
        1997338\\
        71\\
        22\\
        57\\
        1468\\
        766\\
        17\\
        25\\
        995\\
        29\\
        3436\\
        248\\
        72\\
        28\\
        22\\
        3691\\
        2758\\
        28\\
        56\\
        40\\
        30\\
        14\\
        31\\
        47\\
        3522\\
        159\\
        47\\
        14\\
        105\\
        4827\\
        17\\
        84\\
        81\\
        15\\
        728\\
        44\\
        11\\
        59\\
        16\\
        35\\
        341\\
        28\\
        39\\
        94\\
        97\\
        1319\\
        51\\
        10305\\
        75\\
        2336\\
        92\\
        747\\
        22\\
        3274\\
        10\\
        335\\
        238\\
        22\\
        185\\
        601\\
        75\\
        126\\
        227\\
        220\\
        878\\
        142\\
        10\\
        1033\\
        10\\
        305\\
        45\\
        183\\
        4752\\
        16\\
        86\\
        38\\
        730\\
        15\\
        1022\\
        18\\
        372\\
        37\\
        4660\\
        3116\\
        1090\\
        71\\
        720\\
        30\\
        43\\
        186\\
        1551\\
        48\\
        1184\\
        180\\
        164\\
        40\\
        3358\\
        27\\
        1023\\
        1794\\
        125\\
        62\\
        24\\
        35\\
        55\\
        32\\
        201\\
        20\\
        43\\
        25\\
        76\\
        126\\
        1835\\
        38\\
        152\\
        26\\
        16\\
        17\\
        117\\
        12\\
        1662\\
        195\\
        37\\
        54\\
        2040\\
        23\\
        107\\
        9\\
        910\\
        87\\
        465\\
        15\\
        101\\
        9\\
        30\\
        24\\
        26\\
        39\\
        18\\
        96\\
        101\\
        50\\
        1475\\
        1427\\
        1130\\
        66\\
        5732\\
        21\\
        3381\\
        35\\
        89\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.2,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        232\\
        44\\
        110\\
        2528\\
        19\\
        37\\
        26\\
        464\\
        1102\\
        22\\
        11\\
        126\\
        2456\\
        171\\
        6\\
        18\\
        30\\
        2\\
        16\\
        1997305\\
        17\\
        16\\
        22\\
        1412\\
        649\\
        3\\
        16\\
        987\\
        2\\
        1808\\
        242\\
        67\\
        22\\
        17\\
        3628\\
        31\\
        23\\
        7\\
        25\\
        22\\
        8\\
        23\\
        1\\
        3508\\
        107\\
        27\\
        8\\
        73\\
        4238\\
        13\\
        52\\
        31\\
        5\\
        691\\
        21\\
        6\\
        20\\
        0\\
        15\\
        37\\
        18\\
        5\\
        13\\
        92\\
        1229\\
        33\\
        3703\\
        71\\
        1372\\
        54\\
        21\\
        11\\
        3259\\
        1\\
        291\\
        15\\
        8\\
        61\\
        595\\
        60\\
        86\\
        212\\
        10\\
        830\\
        92\\
        3\\
        868\\
        6\\
        5\\
        6\\
        118\\
        4743\\
        4\\
        61\\
        18\\
        520\\
        13\\
        331\\
        5\\
        8\\
        20\\
        95\\
        3051\\
        13\\
        4\\
        331\\
        12\\
        7\\
        146\\
        1493\\
        41\\
        112\\
        157\\
        121\\
        3\\
        1527\\
        23\\
        958\\
        691\\
        89\\
        27\\
        12\\
        26\\
        20\\
        15\\
        195\\
        4\\
        19\\
        7\\
        26\\
        38\\
        1795\\
        31\\
        73\\
        18\\
        1\\
        10\\
        50\\
        5\\
        1580\\
        34\\
        20\\
        28\\
        102\\
        2\\
        81\\
        4\\
        850\\
        21\\
        187\\
        1\\
        77\\
        2\\
        11\\
        11\\
        3\\
        0\\
        4\\
        75\\
        66\\
        19\\
        1444\\
        1342\\
        277\\
        39\\
        12\\
        7\\
        1786\\
        25\\
        48\\
        };
        
        \addplot+[boxplot, 
                  /pgfplots/boxplot/hide outliers, 
                  boxplot/draw direction = y,
                  mark = *,
                  boxplot,
                  fill,fill opacity=0.3,
                  black]
        table[row sep=\\,y index=0] {
        data\\
        9\\
        250\\
        2\\
        7\\
        18\\
        5\\
        326686\\
        71\\
        1584\\
        2\\
        12\\
        20\\
        2\\
        60\\
        59\\
        49\\
        5\\
        65\\
        12\\
        1075885\\
        3\\
        5\\
        1035492\\
        16\\
        288534\\
        264\\
        5\\
        663\\
        10\\
        11\\
        85\\
        559\\
        10\\
        17\\
        26\\
        9\\
        42\\
        550\\
        5\\
        380\\
        7\\
        7\\
        27\\
        12\\
        11\\
        8\\
        118\\
        95\\
        559\\
        317\\
        41\\
        3\\
        5\\
        445\\
        963\\
        3074\\
        1422\\
        182\\
        3475\\
        4009\\
        449\\
        21\\
        3367\\
        323\\
        390\\
        3926\\
        1876\\
        2111\\
        3\\
        427\\
        253\\
        2087\\
        19\\
        952\\
        4\\
        1047\\
        4604127\\
        2\\
        853\\
        1469\\
        334\\
        5\\
        20\\
        2\\
        4\\
        216\\
        150\\
        158067\\
        108\\
        51\\
        533\\
        10\\
        147\\
        5\\
        35\\
        13\\
        1\\
        1\\
        11\\
        71\\
        40\\
        691\\
        5\\
        1740\\
        1041\\
        66\\
        202\\
        804351\\
        9\\
        35\\
        5\\
        92\\
        607533\\
        21\\
        647\\
        148\\
        231\\
        19\\
        113\\
        4\\
        17\\
        22\\
        7\\
        892\\
        784\\
        8\\
        282\\
        11\\
        621\\
        7\\
        2\\
        772\\
        12\\
        9\\
        915\\
        21\\
        1040\\
        621\\
        22\\
        18\\
        3\\
        8\\
        151\\
        6\\
        21\\
        10\\
        4\\
        119\\
        6\\
        186\\
        259\\
        283\\
        1299\\
        1333\\
        27\\
        8\\
        956\\
        104\\
        18\\
        41\\
        7\\
        72\\
        198\\
        6\\
        76\\
        4\\
        26\\
        20\\
        4\\
        129\\
        1293\\
        1\\
        21\\
        39\\
        270\\
        13\\
        67\\
        4\\
        675488\\
        6\\
        1\\
        5\\
        4\\
        64\\
        4\\
        109\\
        47\\
        31\\
        5\\
        76\\
        18\\
        12\\
        3\\
        19\\
        4\\
        11\\
        16\\
        16\\
        17\\
        28\\
        243\\
        5\\
        633\\
        4\\
        422\\
        4\\
        5\\
        10\\
        3091\\
        789\\
        2640\\
        2393\\
        1287\\
        126\\
        1841\\
        3108\\
        3\\
        84\\
        538\\
        1907\\
        46\\
        6\\
        35\\
        50\\
        100\\
        11\\
        1287\\
        38\\
        6\\
        44\\
        39\\
        5\\
        18\\
        1\\
        28\\
        1\\
        4\\
        19\\
        3\\
        4\\
        9\\
        10\\
        6\\
        4\\
        8\\
        62\\
        5\\
        10\\
        2\\
        7\\
        };
        \end{axis}
        \end{tikzpicture}
        }
% \vspace{-2mm}
\caption{Time delay of receiving accepted answer (\texttt{MICO} = Missing Code; \texttt{COAC} = Code After Comment; \texttt{COAC\textsuperscript{*}} = COAC regarding the editing time to add code; \texttt{CODS} = Code During  Submission)}
% \vspace{-3mm}
\label{fig:delay-receiving-acc-ans}
\end{figure}

==> table-false-positive.tex <==

\begin{table*}[!htb]
	\centering
	\captionsetup{justification=centering, labelsep=newline}
	\caption{Summary of false-positive samples}
	\label{table:false-positive}
	\resizebox{6in}{!}{%
    \begin{tabular}{p{4cm}|l|p{12cm}}
    \toprule
    
    \multicolumn{3}{c}{\textbf{Category 1: Questions missed code}} \\ \midrule %file_V1.1_Cat_1
    
    \multicolumn{1}{c|}{\textbf{Reasons}} & \multicolumn{1}{c|}{\textbf{Count (\%)}} & \multicolumn{1}{c}{\textbf{Description}} \\ \midrule
    
     Key phrases were used in different contexts & 114 (42.1\%) &  The comment includes our key phrases. However, they were not meant to ask to add code to questions. Example - \emph{``If I want to \ul{add code} in another web page, for example, a search box, I wanna use my own Ext Core version independently of the version that the user uses''} \citep{keyPhrasesInDifferentContext}   \\ \midrule
     
     Added code as an image file                 & 110 (40.6\%) &  Our program attempts to see whether the questions contain code utilizing the designated HTML tag (e.g., \emph{<pre><code> .... </pre></code>}). However, it fails to find the code snippets when they were included as image files. Example questions -- \citep{addedCodeAsImage1, addedCodeAsImage2}   \\ \midrule
     
     Added an external link to code              & 22  (8.1\%)   & Like the image file, our program fails to find the code snippets when question submitters include external links to code snippets. Example questions -- \citep{addedCodeAsExternalLink1, addedCodeAsExternalLink2}      \\ \midrule
     
     Added code as a comment                     & 18  (6.6\%)  &  Question submitters responded to the comments and added code snippets as comments. Example questions -- \citep{addedCodeAsComment1, addedCodeAsComment2}  \\ \midrule
     
     Self-accepted answer                        & 4   (1.5\%)  & We attempt to find a correlation between question categories and answer meta-data (e.g., presence of accepted answer). To avoid bias, we thus discard the self-accepted questions (i.e., question submitters answered questions \& accepted them). Example question -- \citep{selfAcceptedAnswer} \\ \midrule
     
     Improper code format                        & 3   (1.1\%)  & Code snippets were not included in the appropriate format (e.g., added as plain text) and under the designated HTML tags. Thus our program fails to find the code snippets. Example question -- \citep{improperFormat}  \\ \midrule
     
     
    \multicolumn{3}{c}{\textbf{Category 2: Questions added code after comment}} \\ \midrule %%file_V1.4_Cat_2
    
    Key phrases were used in different contexts   & 168 (53\%) &  -- \\ \midrule
    
    Improper code format                          & 46 (14.5\%)  & Code snippets were included during submission but not in the appropriate format. Example question -- \citep{improperFormatCodeAfterComment} \\ \midrule
    
    Did not follow comments to add code           & 35 (11\%)  & Minimal/inappropriate code snippets were added to the questions. Thus users asked for more/appropriate code snippets. However, question submitters neither follow them nor add the requested code snippets. Example question -- \citep{askedButNotAddedCode} \\ \midrule
    
    Suggested adding code to online code editors  & 23 (7.3\%) & There were code snippets during submission. However, users suggested adding code to online code editors sites such as jsfiddle/codesandbox/stackblitz. Example -- \emph{``Can you add code in jsfiddle?''} \citep{askedToAddCodeJsfiddle} \\ \midrule
    
    Added code as an image file                   & 23 (7.3\%)     & Code snippets were added during submission as an image file. \\ \midrule
    
    Added an external link to code                & 9 (2.8\%)   &  Links to the code snippets were added during submission. \\ \midrule
    
    Self-accepted answer                          & 8 (2.5\%)   &  -- \\ \midrule
    
    Other                                         & 5 1.6\%)    & \ding{117} Added code link. Unfortunately, others found it inactive. 
                                                                \ding{117} Added irrelevant code in response to comments.
                                                                \ding{117} There was a large code during submission. Thus users were asked to add only the relevant parts of the code instead of the complete files because they struggled to find the relevant parts.
                                                                \ding{117} Asked to add compilable code. \\ \midrule
                                                                
    \multicolumn{3}{c}{\textbf{Category 3: Questions added code during submission}} \\ \midrule %file_V1.2_Cat3
    
    No/minimal code during submission          & 53 (57\%)  &   An entire/significant part of code snippets was added later by editing the questions. Example question -- \citep{noCodeDuringSubmission} \\ \midrule
    
    No real code under the designated HTML tag & 39 (41.9\%) &  No real code during submission. Added compiler error message /sample input-output/ stack trace. Example question -- \citep{noRealCodeDuringSubmission} \\ \midrule
    
    Other                                   & 1 (1.1\%) & Added code link. Unfortunately, others found it inactive.  \\ \bottomrule
    \end{tabular}
    }
\end{table*}
